Distilling Drifting Transformers with Representation Autoencoders

Despite the significant training acceleration and promising performance, Representation Autoencoders (RAEs) are mainly criticized for poor distillation effectiveness. In this work, we argue that RAE is competent at high-quality one-step generation. We achieve 1.48 FID with only 16-epoch distillation on ImageNet 256 dataset, surpassing various state-of-the-art methods. To achieve this, we quantitatively study the geometrical behavior of different underlying data spaces. We conclude that conventional distillation methods heavily rely on priors of plain teacher denoising trajectories, while RAE incurs much more complex trajectories with poor properties due to ill anisotropical latent space. We introduce the recently proposed drifting field as the distillation methodology, which makes use of semantically rich RAE latents and provides direct supervision involving no dependency. Bridging our Drift-RAE with previous generative paradigms, we propose several insightful modifications, including the first extrapolation-based guided sampling pipeline for one-step generation with barely no cost. The code will be made publicly available.

==> figs/curvature_panel.tex <==
\includegraphics[width=\linewidth]{figs/compare_curvatures.pdf}

==> sections/7.ack.tex <==
\section*{Acknowledgements}



==> tables/latent_dispersion_table.tex <==
% \small
\begin{tabular}{lcc}
    \toprule
    Latent space & NN-d $(\downarrow)$ & S-MMD $(\uparrow)$ \\
    \midrule
    SD-VAE & 4.3083 & 0.00576 \\
    RAE    & 1.0664 & 0.07913 \\
    \bottomrule
\end{tabular}

==> tables/main_results.tex <==
\begin{table*}[t]
\centering
\caption{
Main results on ImageNet $256\times256$.
$^\dag$ indicates distillation methods. Within each latent space, \textbf{bold} indicates the best result, and \underline{underlining} indicates the second-best result. We highlight the one-step results in color \textcolor{gray}{gray}.
}
\label{tab:main_results}
\footnotesize
\SetTblrInner{rowsep=0.95pt}                     % Row space.
\SetTblrInner{colsep=4.0pt}                      % Col space.
%\begin{adjustbox}{max width=\textwidth}
\begin{tblr}{
    cell{1-42}{2-7}={halign=c,valign=m},         % Text alignment for all cells.
    cell{1-42}{1}={halign=l,valign=m},           % Text alignment for all cells.
    hline{1-3,10,11,24,25,29,30,37}={1-7}{1.0pt},      % Horizontal lines.
    cell{4-9,18-23,32-36}{1-7}={bg=lightgray!35},     % Gray cell color.
}
\textbf{Method}                                            & NFE & Epochs & FID ($\downarrow$) & $\text{FD}_\text{DINOv2}$ ($\downarrow$) & Prec. ($\uparrow$) & Rec. ($\uparrow$) \\
\textbf{Pixel Space}                                       &     &        &                    &                                          &                    &                   \\
ADM-G~\citep{dhariwal2021adm}                              & 250 &    400 &               4.59 &                                       -- &               0.82 &              0.52 \\
BigGAN~\citep{brock2019biggan}                             &   1 &     -- &               6.95 &                                       -- &      \textbf{0.89} &              0.38 \\
GigaGAN~\citep{kang2023gigagan}                            &   1 &    364 &               3.45 &                                       -- &               0.84 &     \textbf{0.61} \\
StyleGAN-XL~\citep{sauer2022styleganxl}                    &   1 &     -- &               2.30 &                                       -- &               0.78 &              0.53 \\
Drifting Model, L/16~\citep{deng2026generative}            &   1 &    640 &   \underline{1.61} &                        \underline{89.84} &   \underline{0.81} &  \underline{0.60} \\
MeanFlow-H/16~\citep{lu2026one}                            &   1 &    320 &               2.29 &                           \textbf{76.96} &               0.80 &              0.59 \\
PaGoDa$^\dag$~\citep{Kim2024pagoda}                        &   1 &     -- &      \textbf{1.56} &                                       -- &                 -- &              0.59 \\
\textbf{SD-VAE}                                            &     &        &                    &                                          &                    &                   \\
DiT-XL/2~\citep{peebles2023dit}                            & 250 &   1400 &               2.27 &                                       -- &      \textbf{0.83} &              0.57 \\
SiT-XL/2~\citep{ma2024sit}                                 & 250 &   1400 &               2.06 &                                   111.86 &   \underline{0.82} &              0.59 \\
IMM-XL/2 ($\omega=1.5$)~\citep{zhou2025inductive}          &   8 &   3837 &               1.99 &                                       -- &                 -- &                -- \\
STEI$^\dag$~\citep{liu2026learning}                        &   8 &     20 &               1.96 &                                       -- &                 -- &                -- \\
MeanFlow-XL/2+~\citep{geng2025meanflow}                    &   2 &   1000 &               2.20 &                                       -- &                 -- &                -- \\
iMF-XL/2~\citep{geng2025improved}                          &   2 &    800 &               1.61 &                           \textbf{89.51} &               0.79 &     \textbf{0.63} \\
$\pi$-Flow$^\dag$~\citep{piflow}                           &   2 &     76 &               1.97 &                                       -- &                 -- &                -- \\
IMM-XL/2 ($\omega=1.5$)~\citep{zhou2025inductive}          &   1 &   3837 &               8.05 &                                       -- &                 -- &                -- \\
MeanFlow-XL/2~\citep{geng2025meanflow}                     &   1 &    240 &               3.43 &                                       -- &                 -- &                -- \\
iMF-XL/2~\citep{geng2025improved}                          &   1 &    800 &               1.82 &                       \underline{103.55} &               0.78 &     \textbf{0.63} \\
Drifting Model, L/2~\citep{deng2026generative}             &   1 &   1280 &   \underline{1.54} &                                   146.88 &               0.79 &     \textbf{0.63} \\
$\pi$-Flow$^\dag$~\citep{piflow}                           &   1 &    448 &               2.85 &                                       -- &                 -- &                -- \\
FreeFlow-XL/2$^\dag$~\citep{tong2025freeflow}              &   1 &    300 &      \textbf{1.45} &                                       -- &                 -- &                -- \\
\textbf{VA-VAE}                                            &     &        &                    &                                          &                    &                   \\
LightningDiT-XL~\citep{Yao2025ReconstructionVG}            & 250 &    800 &   \underline{1.35} &                           \textbf{53.38} &      \textbf{0.79} &     \textbf{0.65} \\
DMD2$^\dag$~\citep{yin2024improved}                        &   2 &      2 &               4.18 &                                       -- &               0.50 &  \underline{0.60} \\
FSF-DMD$^\dag$~\citep{kim2026distribution}                 &   2 &    0.4 &               3.85 &                                       -- &   \underline{0.53} &              0.59 \\
FACM$^\dag$~\citep{peng2026facm}                           &   2 &     60 &      \textbf{1.32} &                                       -- &                 -- &                -- \\
\textbf{RAE}                                               &     &        &                    &                                          &                    &                   \\[2pt]
DiT$^{\mathrm{DH}}$-XL~\citep{zheng2025diffusion}          &  50 &    800 &      \textbf{1.13} &                           \textbf{29.92} &      \textbf{0.78} &     \textbf{0.67} \\
MF-RAE$^\dag$~\citep{hu2025raemeanflow}                    &   2 &     41 &               1.89 &                                       -- &                 -- &                -- \\
MF-RAE$^\dag$~\citep{hu2025raemeanflow}                    &   1 &     41 &               2.03 &                                       -- &                 -- &                -- \\
\method (DiT$^{\mathrm{DH}}$-L)$^\dag$                     &   1 &     16 &               2.10 &                                    57.71 &      \textbf{0.78} &              0.63 \\
\method (DiT$^{\mathrm{DH}}$-L) + IDG$^\dag$               &   1 &     16 &               1.82 &                                    51.81 &      \underline{0.77} &              0.64 \\
\method (DiT$^{\mathrm{DH}}$-XL)$^\dag$                    &   1 &     16 &               1.74 &                                    46.54 &      \textbf{0.78} &              0.64 \\
\method (DiT$^{\mathrm{DH}}$-XL) + IDG $^\dag$             &   1 &     16 &   \underline{1.48} &                        \underline{40.93} &   \underline{0.77} &  \underline{0.66} \\
\end{tblr}
%\end{adjustbox}
\end{table*}



% \begin{table*}[t]
% \centering
% \caption{
% Main results on ImageNet $256\times256$.
% $^\dag$ indicates that the metric reported with guidance.
% }
% \label{tab:main_results}
% \scriptsize
% \SetTblrInner{rowsep=1.25pt}                     % Row space.
% \SetTblrInner{colsep=5.5pt}                      % Col space.
% \begin{tblr}{
%     cell{1-33}{2-8}={halign=c,valign=m},         % Text alignment for all cells.
%     cell{1-33}{1}={halign=l,valign=m},           % Text alignment for all cells.
%     hline{1-3,11,12,26,27,34}={1-8}{1.0pt},      % Horizontal lines.
%     % cell{6-13,20-31}{1-5}={bg=lightgray!35},     % Gray cell color.
% }
% \textbf{Method}                                            & NFE & FDr$^6$ ($\downarrow$) & FID ($\downarrow$) & FD-DINO ($\downarrow$) & IS ($\uparrow$) & Prec. ($\uparrow$) & Rec. ($\uparrow$) \\
% \textbf{Pixel Space}                                       &     &                        &                    &                        &                 &                    &                   \\
% ADM-G$^\dag$~\citep{dhariwal2021adm}                       & 250 &                     -- &               4.59 &                     -- &           186.7 &               0.82 &              0.52 \\
% BigGAN~\citep{brock2019biggan}                             &   1 &                     -- &               6.95 &                     -- &           152.8 &               0.89 &              0.38 \\
% GigaGAN~\citep{kang2023gigagan}                            &   1 &                     -- &               3.45 &                     -- &           225.5 &               0.84 &              0.61 \\
% StyleGAN-XL~\citep{sauer2022styleganxl}                    &   1 &                     -- &               2.30 &                     -- &           265.1 &               0.78 &              0.53 \\
% Drifting Model-L/16~\citep{deng2026generative}             &   1 &                  10.51 &               1.61 &                  89.84 &           307.5 &               0.81 &              0.60 \\
% Pixel MeanFlow-L/16~\citep{lu2026one}                      &   1 &                   9.09 &               2.72 &                  95.04 &           261.7 &               0.81 &              0.56 \\
% Pixel MeanFlow-H/16~\citep{lu2026one}                      &   1 &                   6.87 &               2.29 &                  76.96 &           267.2 &               0.80 &              0.59 \\
% Pixel MeanFlow-L/16+FD-loss~\citep{yang2026representation} &   1 &                   2.09 &               0.78 &                  31.39 &           309.2 &               0.76 &              0.67 \\
% \textbf{SD-VAE}                                            &     &                        &                    &                        &                 &                    &                   \\
% DiT-XL/2$^\dag$~\citep{peebles2023dit}                     & 250 &                     -- &               2.27 &                     -- &           278.2 &               0.83 &              0.57 \\
% SiT-XL/2$^\dag$~\citep{ma2024sit}                          & 250 &                   8.44 &               2.06 &                 111.86 &           270.3 &               0.82 &              0.59 \\
% SiT-XL/2 + REPA$^\dag$~\citep{yu2025repa}                  & 250 &                   5.45 &               1.42 &                  60.62 &           305.7 &               0.80 &              0.65 \\
% IMM-XL/2 ($\omega=1.5$)~\citep{zhou2025inductive}          &   8 &                     -- &               1.99 &                     -- &              -- &                 -- &                -- \\
% Shortcut-XL/2$^\dag$~\citep{frans2025one}                  &   4 &                     -- &               7.80 &                     -- &              -- &                 -- &                -- \\
% iCT-XL/2~\citep{song2024ict}                               &   2 &                     -- &              20.30 &                     -- &              -- &                 -- &                -- \\
% MeanFlow-XL/2$^\dag$~\citep{geng2025meanflow}              &   2 &                     -- &               2.20 &                     -- &              -- &                 -- &                -- \\
% Improved MeanFlow-XL/2~\citep{geng2025improved}            &   2 &                   7.48 &               1.61 &                  89.51 &           289.1 &               0.79 &              0.63 \\
% IMM-XL/2 ($\omega=1.5$)~\citep{zhou2025inductive}          &   1 &                     -- &               8.05 &                     -- &              -- &                 -- &                -- \\
% Shortcut-XL/2$^\dag$~\citep{frans2025one}                  &   1 &                     -- &              10.60 &                     -- &              -- &                 -- &                -- \\
% iCT-XL/2~\citep{song2024ict}                               &   1 &                     -- &              34.24 &                     -- &              -- &                 -- &                -- \\
% MeanFlow-XL/2$^\dag$~\citep{geng2025meanflow}              &   1 &                     -- &               3.43 &                     -- &              -- &                 -- &                -- \\
% Improved MeanFlow-XL/2~\citep{geng2025improved}            &   1 &                   8.39 &               1.82 &                 103.55 &           278.9 &               0.78 &              0.63 \\
% Drifting Model-L/2$^\dag$~\citep{deng2026generative}       &   1 &                  10.92 &               1.54 &                 146.88 &           258.9 &               0.79 &              0.63 \\
% \textbf{RAE}                                               &     &                        &                    &                        &                 &                    &                   \\
% DiT$^{\mathrm{DH}}$-XL~\citep{zheng2025diffusion}          &  50 &                     -- &               1.51 &                  42.04 &           242.9 &               0.79 &              0.63 \\
% DiT$^{\mathrm{DH}}$-XL$^\dag$~\citep{zheng2025diffusion}   &  50 &                   3.26 &               1.13 &                  29.92 &           262.6 &               0.78 &              0.67 \\
% MF-RAE~\citep{hu2025raemeanflow}                           &   2 &                     -- &               1.89 &                     -- &              -- &                 -- &                -- \\
% MF-RAE~\citep{hu2025raemeanflow}                           &   1 &                     -- &               2.03 &                     -- &              -- &                 -- &                -- \\
% \method (DiT$^{\mathrm{DH}}$-L)                            &   1 &                   6.25 &               2.12 &                  57.65 &           218.0 &               0.78 &              0.63 \\
% \method (DiT$^{\mathrm{DH}}$-XL, 10k)                      &   1 &                   5.24 &               1.74 &                  46.11 &           240.2 &               0.78 &              0.63 \\
% \method (DiT$^{\mathrm{DH}}$-XL, 70k)                      &   1 &                   5.27 &               1.72 &                  47.09 &           234.6 &               0.78 &              0.64 \\
% \end{tblr}
% \end{table*}
